Adaptive IGAFEM with optimal convergence rates: Hierarchical B-splines

We consider an adaptive algorithm for finite element methods for the isogeometric analysis (IGAFEM) of elliptic (possibly non-symmetric) second-order partial differential equations in arbitrary space dimension $d\ge2$. We employ hierarchical B-splines of arbitrary degree and different order of smoothness. We propose a refinement strategy to generate a sequence of locally refined meshes and corresponding discrete solutions. Adaptivity is driven by some weighted residual a posteriori error estimator. We prove linear convergence of the error estimator (resp. the sum of energy error plus data oscillations) with optimal algebraic rates. Numerical experiments underpin the theoretical findings.

==> 07_final.tex <==
% !TEX encoding = MacOSRoman
%!TEX root = igafem.tex

%\section{Final remarks}\label{sec:remarks}

%\subsection{\myrev{Optimality of \cite{bg}-algorithm}}
%\myrev{Instead of applying our new proposed mesh-refinement strategy Algorithm~\ref{alg:refinement}, one can also use the strategy of \cite{bg,morgenstern}, see Remark~\ref{rem:morgenstern}.
%In this case, one has to use a different definition of admissibility \cite[Definition 10]{bg}:
%We call a hierarchical mesh $\TT_\bullet$ admissible\footnote{Eigentlich zeigen sie nicht, dass  ihr $\refine$ genau  die feineren strictly admissible meshes ergibt. Das braucht man aber nicht wirklich...} if it is strictly admissible in the sense of \cite{bg,morgenstern}, see  Remark~\ref{rem:morgenstern}.
%%In \cite{bg,morgenstern}, these meshes are actually refered to as strictly admissible, see also Remark~\ref{rem:morgenstern}.%all truncated hierarchical B-splines $\set{\Trunc_\bullet(\beta)}{\beta\in\HH_\bullet}$ which take non-zero values over any element $T\in\TT_\bullet$ belong to at most two successive levels.
%The set of all admissible meshes is again denoted by $\T$.
%Then, the main result Theorem~\ref{thm:main} holds true as well.
%Here, we note that reliability and linear convergence has already been proved in \cite{bg}.
%By \cite[Section 2.4]{bg} their strategy satisfies \eqref{M:shape}--\eqref{M:trace}.
%The mesh-refinement properties \eqref{R:sons}--\eqref{R:overlay} have been proved in \cite{morgenstern}.
%\eqref{S:inverse}--\eqref{S:nestedness} follow along the lines of  Section \ref{subsec:E1.1 true}--\ref{subsec:nestedness}.
%Indeed, the only new and challenging part is the verification of \eqref{S:local}--\eqref{S:grad}.
%If one goes carefully through the corresponding proofs, see Section~\ref{subsec:E4.2 true}--\ref{subsec:E4.1 true}, one sees that the key argument the existence of some $k\in\N_0$ such that $T\subseteq\supp(\beta)$ implies $\supp(\beta)\subseteq\pi_\bullet^k(T)$ for all $T\in\TT_\bullet, \beta\in\HH_\bullet$.
%%However, \eqref{eq:grad trunc} remains valid\footnote{Vermutlich?!...} for the strategy of \cite{morgenstern}.
%However, this  argument  holds as well\footnote{Vermutlich?!...} for $\Trunc_\bullet(\beta)$ instead of $\beta$.
%As in the previous Section~\ref{subsec:rational}, one sees that one could  even use rational hierarchical splines $\XX_\bullet^{W_0}$ as ansatz space.
%}

